Causal inference methods for combining randomized trials and observational studies: a review

With increasing data availability, causal effects can be evaluated across different data sets, both randomized controlled trials (RCTs) and observational studies. RCTs isolate the effect of the treatment from that of unwanted (confounding) co-occurring effects but they may suffer from unrepresentativeness, and thus lack external validity. On the other hand, large observational samples are often more representative of the target population but can conflate confounding effects with the treatment of interest. In this paper, we review the growing literature on methods for causal inference on combined RCTs and observational studies, striving for the best of both worlds. We first discuss identification and estimation methods that improve generalizability of RCTs using the representativeness of observational data. Classical estimators include weighting, difference between conditional outcome models, and doubly robust estimators. We then discuss methods that combine RCTs and observational data to either ensure uncounfoundedness of the observational analysis or to improve (conditional) average treatment effect estimation. We also connect and contrast works developed in both the potential outcomes literature and the structural causal model literature. Finally, we compare the main methods using a simulation study and real world data to analyze the effect of tranexamic acid on the mortality rate in major trauma patients. A review of available codes and new implementations is also provided.

==> ipswShuYang.tex <==

%% Shu Yang part
To overcome this bias, most existing methods rely on direct modeling of the sampling score
previously introduced.  The sampling score adjustments methods include inverse probability
of sampling weighting (IPSW; \citealp{cole2010generalizing,buchanan2018generalizing}) and
stratification \citep{tipton2013improving,o2014generalizing}.
Most of the
empirical literature assumes that $\pi_{ S}(X)$ follows a logistic
regression model and can be estimated by
$\widehat\pi_{ S}(X)$. 


We consider various parametric and nonparametric methods to estimate
the sampling score. For parametric approaches, we first assume the target
population size $N$ is known. Similar to most of the empirical literature,
we can posit a logistic regression model for $\pi_{S}(X)$; i.e.,
$\logit\{\pi_{S}(X;\alpha)\}=\alpha_{0}+\alpha_{1}^{\intercal}X$,
where $\alpha=(\alpha_{0},\alpha_{1}^{\intercal})^{\intercal}\in\mathbb{R}^{p+1}$.
The typical maximum likelihood estimator of $\alpha$ can be obtained
by 
\begin{align}
\widehat{\alpha}= & \underset{\alpha}{\mathrm{argmax}}\frac{1}{N}\sum_{i=1}^{N}\left[S_{i}(\alpha_{0}+\alpha_{1}^{\intercal}X_{i})-\mathrm{log}\left\{ 1+\mathrm{exp}(\alpha_{0}+\alpha_{1}^{\intercal}X_{i})\right\} \right].\label{eq:mle}
\end{align}
However, the second term $N^{-1}\sum_{i=1}^{N}\mathrm{log}\left\{ 1+\mathrm{exp}(\alpha_{0}+\alpha_{1}^{\intercal}X_{i})\right\} $
in (\ref{eq:mle}) is not feasible to calculate because we can not
observe $X$ for all individuals in the population. The key insight
is that this term can be estimated by $m^{-1}\sum_{i=n+1}^{n+m}\mathrm{log}\left\{ 1+\mathrm{exp}(\alpha_{0}+\alpha_{1}^{\intercal}X_{i})\right\} $
based on the observational sample. This strategy leads to our modified maximum likelihood
estimator
\begin{equation}
\widehat{\alpha}=\underset{\alpha}{\mathrm{argmax}}\left[\frac{1}{N}\sum_{i=1}^{N}S_{i}(\alpha_{0}+\alpha_{1}^{\intercal}X_{i})-\frac{1}{m}\sum_{i=1}^{m}\mathrm{log}\left\{ 1+\mathrm{exp}(\alpha_{0}+\alpha_{1}^{\intercal}X_{i})\right\} \right].\label{eq:ee0}
\end{equation}
\jp{Shouldn't we also replace $N$ by $n$ in the first term?}
Alternatively, for any $g(X),$ we have
\begin{equation}
\E\left[\frac{Sg(X)}{\pi_{S}(X)}\right]=\E\left[g(X)\right].\label{eq:bal}
\end{equation}
Therefore, we can use the following estimating equations 
\begin{equation}
\frac{1}{N}\sum_{i=1}^{N}\frac{S_{i}g(X_{i})}{\pi_{S}(X_{i};\alpha)}=\frac{1}{m}\sum_{i=n+1}^{n+m}g(X_{i})\label{eq:ee1}
\end{equation}
for $\alpha$, where $g(X)\in\mathbb{R}^{p+1}$. For simplicity, one
can take $g(X)$ as $\partial\logit\{\pi_{S}(X;\alpha)\}/\partial\alpha$.
Optimal form of $g(X)$ is also available from the literature. Equations (\ref{eq:ee0}) and 
(\ref{eq:ee1}) requires the population size $N$ to be known. If
$N$ is unknown, we replace $N$ in (\ref{eq:ee0}) and (\ref{eq:ee1}) by $\widehat{N}(\alpha)=\sum_{i=1}^{n}\{\pi_{S}(X_{i};\alpha)\}^{-1}$.
The balance condition (\ref{eq:bal}) also motivates the calibration
weighting approach in Section \ref{sec: CWmethod}. 

\paragraph{Inverse probability of sampling weighting (IPSW)}

The IPSW approach can be seen as the counterpart of inverse propensity weighting (IPW) methods to estimate the ATE from observational studies to control for confounding (see Appendix \ref{sec:appipw} for details). 
Based on the identification formula a), the IPSW estimator of the ATE is defined as the weighted difference of average outcomes between the treated and control group in the trial. The observations are weighted by the inverse of the estimated sampling
score to account for the shift of the covariate distribution from
the RCT sample to the target population: 

\begin{equation}
\label{eq:ipsw}
\widehat{\tau}^{\ipsw}=\frac{\sum_{i=1}^{n}\widehat\pi_{ S}(X_i)^{-1}A_{i}Y_{i}}{\sum_{i=1}^{n}\widehat\pi_{ S}(X_i)^{-1}A_{i}}-\frac{\sum_{i=1}^{n}\widehat\pi_{ S}(X_i)^{-1}(1-A_{i})Y_{i}}{\sum_{i=1}^{n}\widehat\pi_{ S}(X_i)^{-1}(1-A_{i})}.
\end{equation}


%Non normalized formula: \bc{To be confirmed}
%\begin{equation}
%\label{eq:ipswnonnormalized}
%\widehat{\tau}^{\ipsw}= \frac{2}{n+m} \sum_{i=1}^{n} \frac{ A_{i}Y_{i}}{ \widehat\pi_{S}(X_i) } - \frac{ (1-A_{i})Y_{i}}{\widehat\pi_{S}(X_i) }.
%\end{equation}


  The IPSW estimator is consistent when the sampling score is consistently estimated.  \cite{dahabreh2019generalizing} show that it is asymptotically normal and give a consistent sandwich-type
variance estimator. 
Non-parametric bootstrap can also be used to estimate the variance. 
Similar to IPW estimators, IPSW estimators are known to be highly unstable, especially when the sampling scores are extreme. It happens when the observational study contains units with very small probabilities of being in the sample. Normalized weights as in equation \ref{eq:ipsw}, so that they sum to 1, can be used to overcome this issue \citep{dahabreh2019extending}. Still, the major challenge is that IPSW estimators require a correct model specification of the sampling score.  
Avoiding this problem requires either very strong domain expertise or turning to doubly robust methods (Section~\ref{sec:DR}).


==> sections/notations.tex <==
\section{[JP] Attempt to improve / clean notations}
\subsection{Why?}
I found several inconsistencies in the definitions and notations in the paper, probably because different papers we review use slightly different settings. In particular, how the distributions in RCT and RWE are defined. For example:
\begin{itemize}
    \item \citet{dahabreh2018generalizing} model (like us) $\delta$ as indicator variable for RCT ($\delta=1$) and RWE ($\delta=0$), but consequently define the ATE as the average treatment effect on the RCT and RWE population. This is probably not what we want (we say that we are interested in RWE only). Consequently their IPSW formula is not correct for us (that's why BC did not manage to proof S2).
    \item \citet{dong2020integrative} models both RCT and RWE as derived from a common superpopulation with distribution $P$, with random variables $\delta$ and $\tilde{\delta}$ to indicate when a sample from the superpopulation is selected to be in the RCT (with distribution $P$ conditioned to $\delta=1$) or in the RWE (with distribution $P$ conditioned to $\tilde{\delta}=1$). The ATE is defined as the average treatment over the superpopulation (that follows $P$). This is a nice setting, but perhaps we do not want to differentiate the superpopulation and RWE, to simplify notations. \jj{yes, exactly, we start with this one and then want to simplify not to separate RWE and superpopulation}
\end{itemize}

In order to clarify the setting and make sure all formulas are correct, I propose below a (hopefully) coherent set of notations and hypotheses, with corresponding formulas for the various estimators. Basically I take the model of \citet{dong2020integrative} with $P(\tilde{\delta}=1)=1$, i.e., RWE represents the surpopulation on which we want to estimate the average treatment effect, and RCT samples are sampled from the superpopulation and kept only when a binary random variable $S$ is equal to $1$ (I use $S$ like "Selected" instead of $\delta$ since I prefer to be coherent and use upper cases for random variables...). In other words, RCT samples follow $P$ conditioned to $S=1$, while RWE samples follow $P$.

Once we agree they are correct and what we want, we can update the manuscript accordingly.. \jj{Yes, I agree with this setting, thank you very much}


\subsection{Setting and notations}
To model each patient in the RCT or RWE populations, we consider a distribution $P$ over a random tuple $(X,Y(0),Y(1),A,S)$, where $X$ is a $p$-dimensional vector of covariates, $A$ denotes the binary treatment assignment (with $A=0$ for the control and $A=1$ for the treated patients), $Y(a)$ is the binary or continuous outcome had the subject been given treatment $a$ (for $a\in\{0,1\}$), and $S$ in a binary indicator for the inclusion in the RCT ($S=1$) or not ($S=0$). Assuming \emph{consistency of potential outcomes}, we also denote by $Y=AY(1)+(1-A)Y(0)$ the outcome realized under treatment $A$. We model the patients in an RCT sample of size $n$ and in a RWE sample of size $m$ by $n+m$ independent random tuples $(X_i,Y_i(0),Y_i(1),A_i,S_i)_{i=1,\ldots,n+m}$, where the RCT samples $i=1,\ldots,n$ are identically distributed according to $P(X,Y(0),Y(1),A,S \mid S=1)$, and the RWE samples $i=n+1,\ldots,n+m$ are identically distributed according to $P(X,Y(0),Y(1),A,S)$. For each RCT sample $i=1,\ldots,n$, we observe $(X_i,A_i,Y_i,S_i=1)$, while for RWE $i=n+1,\ldots,n+m$, we consider two settings: (i) either we only observe the covariates $X_i$, (ii) or we also observe the treatment and outcome $(X_i,A_i,Y_i)$.

Assuming the RWE samples represent the population of interest, our goal is to estimate the conditional average treatment effect (CATE):
$$
\forall x\in\R^p\,,\quad \tau(x) = \EE [Y(1) - Y(0) \mid X=x]\,,
$$
or simply the population average treatment effect (ATE):
$$
\tau_0 = \EE [Y(1) - Y(0)] = \EE[\tau(X)]\,.
$$
We note that in general, if the samples in the RCT and RWE do not follow the same distribution, then the ATE is different from the RCT average treatment effect:
$$
\tau_0 \neq \tau_1 = \EE [Y(1) - Y(0) \mid S=1]\,.
$$
We denote respectively by $e(x)$ and $e_1(x)$ the propensity score in the RWE and in the RCT population:
$$
e(x) = P(A=1 \mid X=x)\,,\quad e_1(x) = P(A=1 \mid X=x, S=1)\,,
$$
and by $\pi(x)$ the sampling propensity score \citep{tipton2013improving}:
$$
\pi(x) = P(S=1 \mid X=x)\,.
$$

\subsection{Assumptions}

\subsection{Identification formulas}
\begin{itemize}
    \item Reweighting formula:
    \begin{equation}
        \tau_0 = \EE [ \frac{S \tau(X)}{\pi(X)}]\,.
    \end{equation}
    \item Regression formula:
    \begin{equation}
        \tau_0 = \EE [\EE [ Y \mid X, A=1, S=1] ] - \EE [\EE [ Y \mid X, A=0, S=1] ]\,,
    \end{equation}
    where the outer expectations are with respect to $X$.\jp{Note that compared to (2), the conditioning on $\delta=0$ has disappeared in (S4).}
\end{itemize}

\subsection{Estimators}
TODO: correct the formulas to make sure they are correct in our setting. This is currently not the case, for example the IPSW formula should be the one of \citet{dong2020integrative} and not the one of \citet{dahabreh2018generalizing}... TODO


Dong formula added following JPV arguments: 
\begin{equation}
\hat{\tau}^{\ipsw}=\frac{\sum_{i=1}^{n}\pi(X_{i};\widehat{\bEta})^{-1}A_{i}Y_{i}}{\sum_{i=1}^{n}\pi(X_{i};\widehat{\bEta})^{-1}A_{i}}-\frac{\sum_{i=1}^{n}\pi(X_{i};\widehat{\bEta})^{-1}(1-A_{i})Y_{i}}{\sum_{i=1}^{n}\pi(X_{i};\widehat{\bEta})^{-1}(1-A_{i})}.
\end{equation}



==> table_with_hypothesis.tex <==
\begin{table}[h!]
\caption{\textbf{Treatment effect estimators and their characteristics} for RCT, observational data, and combining both data (in the case of non-nested design). GLM: parametric model(s); GRF: non-parametric model(s); CC: complete cases; MI: multiple imputation; C: consistency \eqref{a:consist}; U: unconfoundedness \eqref{a:ign}; UdM: unconfoundedness despite missingness \citep{mayer2019doubly}; O: overlap/positivity of treatment assignment; PT: positivity of trial participation \eqref{a:pos}; T: transportability \eqref{a:trans-3}; R: trial randomization \eqref{a:ign}.}
\label{tab:estimators}
\footnotesize
\begin{tabular}{|l|l||c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Estimator} & \multirow{2}{*}{Model(s)} & \multicolumn{1}{c|}{\multirow{2}{*}{RCT}} & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell[c]{Observational\\data}}}    & \multicolumn{3}{c|}{Missing covariates}  & \multicolumn{2}{c|}{\makecell[c]{Robustness to model\\ mis-specification}}   & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell[c]{Parametric\\convergence\\rate}}} \\
%
 &    & \multicolumn{1}{c|}{}  &  \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\tiny MCAR} & \multicolumn{1}{c|}{\tiny MAR} & \multicolumn{1}{c|}{\tiny MNAR} & \multicolumn{1}{c|}{\tiny\makecell[c]{1 mis-spec.\\ model}} & \multicolumn{1}{c|}{\tiny\makecell[c]{2 mis-spec.\\ models}} & \multicolumn{1}{c|}{}  \\ \hline
%
%
\makecell[l]{Difference in\\means}  &  --  &  \cmark   &   \xmark   &  \cmark   & \cmark  &   \cmark   &  --   &  --  &  \cmark  \\ \hline
%\multirow{2}{*}{\makecell[l]{Difference in\\conditional\\means}} &   \makecell[l]{GLM/\\(+CC)}   &  \cmark    & \makecell[c]{\cmark\\\tiny if C+U+O} &  \cmark    &  \xmark &  \xmark   &  \makecell[c]{\cmark\\\tiny on RCT}    &   --  &   \cmark  \\ \cline{2-10} 
%
% & \makecell[l]{GLM/\\+MI} &  \cmark  &  \makecell[c]{\cmark\\\tiny if C+U+O}  &  \cmark  & \cmark &  \xmark &  \makecell[c]{\cmark\\\tiny on RCT}  &  --  &           \cmark  \\ \hline\hline
%
%
\multirow{3}{*}{IPW} &  \makecell[l]{GLM\\(+CC)}   &  \cmark   &  \makecell[c]{\cmark\\\tiny if C+U+O}  &  \cmark    &  \xmark    &   \xmark   &   \xmark   &  --   &  \cmark \\ \cline{2-10} 
%
 &  \makecell[l]{GLM\\+MI}  &  \cmark  & \makecell[c]{\cmark\\\tiny if C+U+O}  &   \cmark  &  \xmark  &  \xmark  &   \xmark  &  --  &   \cmark   \\ \cline{2-10} 
 &  \makecell[l]{GRF\\(+MIA)}  & \cmark  &  \makecell[c]{\cmark\\\tiny if C+U+O}  & \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U} &  \cmark  & --  &  \xmark   \\ \hline
%
%
\multirow{3}{*}{AIPW} & \makecell[l]{GLM\\(+CC)} &  \cmark  &  \makecell[c]{\cmark\\\tiny if C+U+O} & \cmark  &  \xmark  & \xmark  &   \cmark  &  \xmark   &  \cmark \\ \cline{2-10} 
 & \makecell[l]{GLM\\+MI} &  \cmark  &  \makecell[c]{\cmark\\\tiny if C+U+O}  &   \cmark   &  \cmark  &  \xmark &  \cmark  &  \xmark  & \cmark  \\ \cline{2-10} 
 & \makecell[l]{GRF\\(+MIA)}  &  \cmark   &  \makecell[c]{\cmark\\\tiny if C+U+O}   &  \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  & \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \cmark  &   \cmark   &   \makecell[c]{\cmark\\\tiny if $n^{1/4}$ rate\\\tiny nuisance\\\tiny estimators} \\ \hline\hline
%
%
\multirow{3}{*}{IPSW} &    \makecell[l]{GLM\\(+CC)}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  & \cmark    &  \xmark &  \xmark &   & -- & \\ \cline{2-10} 
 & \makecell[l]{GLM\\+EM}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}   & \cmark  &  \cmark &  \xmark &  \xmark & --  &   \\ \cline{2-10} 
 &  \makecell[l]{GRF\\(+MIA)}  &   \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &   &   &   &   & --  &   \\ \hline
%
\multirow{3}{*}{G-formula} &  \makecell[l]{GLM\\(+CC)}  &  \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}   &  \cmark    &  \xmark &  \xmark  &   & --  &   \\ \cline{2-10} 
 & \makecell[l]{GLM\\+EM}  &  \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &   &   &   &   & --  &   \\ \cline{2-10} 
 & \makecell[l]{GRF\\(+MIA)}   & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &   &   &   &   & --  &   \\ \hline
%
\multirow{3}{*}{AIPSW} &   \makecell[l]{GLM\\(+CC)}   &  \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &  \cmark    &  \xmark &  \xmark  &   &   &   \\ \cline{2-10} 
 &  \makecell[l]{GLM\\+EM}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &  &  &  &  &  &  \\ \cline{2-10} 
 & \makecell[l]{GRF\\(+MIA)}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &  &  &  &  &  &   \\ \hline
\end{tabular}
\end{table}


\subsection{Estimators used in the data analysis section, with their assumptions}

Table~\ref{tab:estimators} recalls all the estimators used in the data analysis, with their assumptions. This table highlights the complexity and variety of underlying assumptions mixing both the transportability topics and the missing data domain.

\begin{table}[t!]
\caption{\textbf{Treatment effect estimators and their characteristics} for RCT, observational data, and combining both data (in the case of non-nested design). GLM: parametric model(s); GRF: non-parametric model(s); CC: complete cases; MI: multiple imputation; C: consistency \eqref{a:consist}; U: unconfoundedness \eqref{a:ign}; UdM: unconfoundedness despite missingness \citep{mayer2019doubly}; O: overlap/positivity of treatment assignment; PT: positivity of trial participation \eqref{a:pos}; T: transportability \eqref{a:trans-3}; R: trial randomization \eqref{a:ign}. The (\cmark) indicates conjectured behaviour but that needs further theoretical investigation.}
\label{tab:estimators}
\footnotesize
\begin{tabular}{|l|l||c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Estimator} & \multirow{2}{*}{Model(s)} & \multicolumn{1}{c|}{\multirow{2}{*}{RCT}} & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell[c]{Observational\\data}}}    & \multicolumn{3}{c|}{Missing covariates}  & \multicolumn{2}{c|}{\makecell[c]{Robustness to model\\ mis-specification}}   & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell[c]{Parametric\\convergence\\rate}}} \\
%
 &    & \multicolumn{1}{c|}{}  &  \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\tiny MCAR} & \multicolumn{1}{c|}{\tiny MAR} & \multicolumn{1}{c|}{\tiny MNAR} & \multicolumn{1}{c|}{\tiny\makecell[c]{1 mis-spec.\\ model}} & \multicolumn{1}{c|}{\tiny\makecell[c]{2 mis-spec.\\ models}} & \multicolumn{1}{c|}{}  \\ \hline
%
%
\makecell[l]{Difference in\\means}  &  --  &  \cmark   &   \xmark   &  \cmark   & \cmark  &   \cmark   &  --   &  --  &  \cmark  \\ \hline
%\multirow{2}{*}{\makecell[l]{Difference in\\conditional\\means}} &   \makecell[l]{GLM/\\(+CC)}   &  \cmark    & \makecell[c]{\cmark\\\tiny if C+U+O} &  \cmark    &  \xmark &  \xmark   &  \makecell[c]{\cmark\\\tiny on RCT}    &   --  &   \cmark  \\ \cline{2-10} 
%
% & \makecell[l]{GLM/\\+MI} &  \cmark  &  \makecell[c]{\cmark\\\tiny if C+U+O}  &  \cmark  & \cmark &  \xmark &  \makecell[c]{\cmark\\\tiny on RCT}  &  --  &           \cmark  \\ \hline\hline
%
%

\multirow{3}{*}{AIPW} & \makecell[l]{GLM\\(+CC)} &  \cmark  &  \makecell[c]{\cmark\\\tiny if C+U+O} & \cmark  &  \xmark  & \xmark  &   \cmark  &  \xmark   &  \cmark \\ \cline{2-10} 
 & \makecell[l]{GLM\\+MI} &  \cmark  &  \makecell[c]{\cmark\\\tiny if C+U+O}  &   \cmark   &  \cmark  &  \xmark &  \cmark  &  \xmark  & \cmark  \\ \cline{2-10} 
 & \makecell[l]{GRF\\(+MIA)}  &  \cmark   &  \makecell[c]{\cmark\\\tiny if C+U+O}   &  \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  & \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \makecell[c]{\cmark\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \cmark  &   \cmark   &   \makecell[c]{\cmark\\\tiny if $n^{1/4}$ rate\\\tiny nuisance\\\tiny estimators} \\ \hline\hline
%
%
\multirow{3}{*}{IPSW} &    \makecell[l]{GLM\\(+CC)}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  & (\cmark)    &  \xmark &  \xmark &  \xmark & -- & \\ \cline{2-10} 
 & \makecell[l]{GLM\\+EM}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}   & (\cmark)  &  (\cmark) &  \xmark &  \xmark & --  &   \\ \cline{2-10} 
 &  \makecell[l]{GRF\\(+MIA)}  &   \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &  \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U} & \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U} &  \xmark  & --  &   \\ \hline
%
\multirow{3}{*}{G-formula} &  \makecell[l]{GLM\\(+CC)}  &  \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}   &  (\cmark)    &  \xmark &  \xmark  & \xmark  & --  &   \\ \cline{2-10} 
 & \makecell[l]{GLM\\+EM}  &  \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &  (\cmark) &  \cmark & \xmark  & \xmark  & --  &   \\ \cline{2-10} 
 & \makecell[l]{GRF\\(+MIA)}   & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  & \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U}  & \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U}  &  \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U} & \xmark & --  &   \\ \hline
%
\multirow{3}{*}{AIPSW} &   \makecell[l]{GLM\\(+CC)}   &  \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  &  (\cmark)    &  \xmark &  \xmark  &   \cmark & \xmark  &   \\ \cline{2-10} 
 &  \makecell[l]{GLM\\+EM}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  & (\cmark) & (\cmark) & \xmark & \cmark & \xmark &  \\ \cline{2-10} 
 & \makecell[l]{GRF\\(+MIA)}  & \multicolumn{2}{c|}{\makecell{\cmark\\\tiny if C+R+T+PT}}  & \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U} &  \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U} & \makecell[c]{(\cmark)\\\tiny if UdM\\\tiny instead\\\tiny of U}  & \cmark & (\cmark) &   \\ \hline
\end{tabular}
\end{table}


